Don't Retrain, Just Rewrite: Countering Adversarial Perturbations by Rewriting Text

Can language models transform inputs to protect text classifiers against adversarial attacks? In this work, we present ATINTER, a model that intercepts and learns to rewrite adversarial inputs to make them non-adversarial for a downstream text classifier. Our experiments on four datasets and five attack mechanisms reveal that ATINTER is effective at providing better adversarial robustness than existing defense approaches, without compromising task accuracy. For example, on sentiment classification using the SST-2 dataset, our method improves the adversarial accuracy over the best existing defense approach by more than 4% with a smaller decrease in task accuracy (0.5% vs 2.5%). Moreover, we show that ATINTER generalizes across multiple downstream tasks and classifiers without having to explicitly retrain it for those settings. Specifically, we find that when ATINTER is trained to remove adversarial perturbations for the sentiment classification task on the SST-2 dataset, it even transfers to a semantically different task of news classification (on AGNews) and improves the adversarial robustness by more than 10%.

==> tables/main_results.tex <==
\begin{table*}[!ht]
\centering
% \begin{tabular}{@{}lrrrrrr@{}}
\begin{tabular}{lccccccr}
\toprule
\textbf{Defense} & \multicolumn{2}{c}{\textbf{SST-2}}                                                                        & \multicolumn{2}{c}{\textbf{Rotten Tomato}}                                                                           & \multicolumn{2}{c}{\textbf{AGNews}}                                                                       &
\textbf{Average} \\ \midrule
                (TextFooler) & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.\end{tabular} \\
 \cmidrule(lr){2-8}
None             & 92.4 & 4.8 & 84.2 & 10.7 & 94.2  & 18.1 & 11.2 \\
\hdashline
Adv.-DA          & 88.4 & 5.7 & 84.2  & 11.3 & -    & -    & 8.5 \\
SHIELD           & 88.8 & 6.6 & 82.1  & 12.1 & -    & -    & 9.3 \\
SAFER            & 89.3 & 8.7 & 85.5  & 3.7  & -    & -    & 6.2 \\
SampleShielder   & 85.0 & 11.3 & 76.3 & 12.1 & 90.8 & 52.6 & 11.7\\
ADFAR            & 89.9 & 19.5 & 82.4 & 17.5 & -    & -    & 18.5 \\
T5-RW (Ours)     & 92.0 & \textbf{24.0}$\uparrow$ & 84.3 & \textbf{21.1}$\uparrow$ & 94.0 & \textbf{57.7}$\uparrow$ & \textbf{34.6}$\uparrow$ \\ \bottomrule
\end{tabular}
\caption{\textbf{Results comparing model robustness using the clean accuracy (\%) and adversarial accuracy (\%) on the TextFooler attack}: Using a vanilla BERT model, we compare using several defense techniques. None indicates the vanilla BERT model without any additional defense mechanism applied and therefore acts as a baseline model for text classification across all datasets. Our model yields state-of-the-art results across the board without losing clean accuracy points.}
\end{table*}




==> tables/main_results_expanded.tex <==
\begin{table*}[!ht]
\centering
% \begin{tabular}{@{}lrrrrrr@{}}
% \small
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccr}
\toprule
\textbf{Defense} & \multicolumn{3}{c}{\textbf{SST-2}}                                                                        & \multicolumn{3}{c}{\textbf{Rotten Tomatoes}}                                                                           & \multicolumn{3}{c}{\textbf{AGNews}}                                                                       &
\textbf{Average} \\ \midrule
                 & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Num. \\ Queries $\uparrow$\end{tabular}  & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Num. \\ Queries $\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Clean \\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Num. \\ Queries $\uparrow$\end{tabular} & \begin{tabular}[c]{@{}r@{}}Adv.\\ Acc.\end{tabular} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
None             & \first{92.4} & 4.8 & 88.2& 84.2 & 10.7 & 99.3& \first{94.9}  & 18.2 & 334.1& 11.2 \\
\hdashline
Adv.-DA          & 88.4 & 5.7 & 91.6 & 84.2  & 11.3 & 99.9& -    & -    & & 8.5 \\
SHIELD           & 88.8 & 6.6 & 90.9& 82.1  & 12.1 & 98.7& -    & -    & & 9.3 \\
SAFER            & 89.3 & 8.7 & 91.9& \first{85.5}  & 3.7  & 88.1& 91.2    & 15.7    & 280.6 & 6.2 \\
SampleShielder   & 85.0 & 11.3 & 100.7 & 76.3 & 12.1 & 105.5& 90.8 & 52.6 & \second{425.6}& 11.7\\
ADFAR            & 89.9 & \second{19.5} & \second{115.4}& 82.4 & \second{17.5} & \second{120.5}& 92.4    & \second{58.3}    & 422.2& 18.5 \\
T5-RW (Ours)     & \second{92.0} & \first{24.0} & \first{136.7}& \second{84.3} & \first{21.1}& \first{140.2}& \second{94.7} & \first{73.0}& \first{520.0}& \textbf{34.6} \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Results comparing model robustness using the clean accuracy (\%) and adversarial accuracy (\%) on the TextFooler attack}: Using a vanilla BERT model, we compare using several defense techniques. None indicates the vanilla BERT model without any additional defense mechanism applied and therefore acts as a baseline model for text classification across all datasets. Our model yields state-of-the-art results across the board without losing clean accuracy points. \textbf{Key:} Elements colored in \first{red} and \second{blue}  mark the best and second-best numbers in their respective columns.}
\label{tab:resultsMain}
\end{table*}


